Measurement of the CP-violation parameter of B^0 mixing and decay with pp(bar) -> mu mu X data

We measure the dimuon charge asymmetry A in pp(bar) collisions at a center of mass energy sqrt{s} = 1960 GeV. The data was recorded with the D0 detector and corresponds to an integrated luminosity of approximately 1.0 fb-1. Assuming that the asymmetry A is due to asymmetric B^0 <-> B(bar)^0 mixing and decay, we extract the CP-violation parameter of B^0 mixing and decay: Re(epsilon_B^0)(1 + |epsilon_B^0|^2) = A_B^0/4 = -0.0023 +/- 0.0011 (stat) +/- 0.0008 (syst). A_B^0 is the dimuon charge asymmetry from decays of B^0 B(bar)^0 pairs. The general case, with CP violation in both B^0 and B_s^0 systems, is also considered. Finally we obtain the forward-backward asymmetry that quantifies the tendency of mu+ to go in the proton direction and mu- to go in the anti-proton direction. The results are consistent with the standard model and constrain new physics.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            8/31/06
%
\bibitem[*]{kurca}
On leave from IEP SAS Kosice, Slovakia.
\bibitem[\dag]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
%\bibitem[\ddag]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA
%
\vskip 0.25cm

